Optimistic Aborts for Geo-distributed Transactions

Network latency can have a significant impact on the performance of transactional storage systems, particularly in wide area or geo-distributed deployments. To reduce latency, systems typically rely on a cache to service read-requests closer to the client. However, caches are not effective for write-heavy workloads, which have to be processed by the storage system in order to maintain serializability. This paper presents a new technique, called optimistic abort, which reduces network latency for high-contention, write-heavy workloads by identifying transactions that will abort as early as possible, and aborting them before they reach the store. We have implemented optimistic abort in a system called Gotthard, which leverages recent advances in network data plane programmability to execute transaction processing logic directly in network devices. Gotthard examines network traffic to observe and log transaction requests. If Gotthard suspects that a transaction is likely to be aborted at the store, it aborts the transaction early by re-writing the packet header, and routing the packets back to the client. Gotthard significantly reduces the overall latency and improves the throughput for high-contention workloads.

==> Makefile <==
PAPER = main
VERBOSE = 0

# directories
FIGURE_DIR = .
OUTPUT_DIR = .
STYLE_DIR = .
TEXT_DIR = .
BIB_OUT_FILE = $(OUTPUT_DIR)/bib-issues

# paths
BIB_PATH="$(TEXT_DIR)"
BST_PATH="$(STYLE_DIR)/sty:$(shell kpsewhich --progname=latex --show-path=.bst)"
TEX_PATH="$(TEXT_DIR):$(STYLE_DIR):$(STYLE_DIR)/sty:$(shell kpsewhich -progname=tex -show-path=tex)"

# options
BIBTEX_OPTS = -terse
DVIPS_OPTS = -q -G0 -tletter
LATEX_OPTS  = -output-directory=$(OUTPUT_DIR) -file-line-error -interaction=batchmode 
MAKEINDEX_OPTS = -q
PS2PDF_OPTS = -q -sPAPERSIZE=letter -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress \
              -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true 

#commands
LATEXC = max_print_line=1000 pdflatex
PRINT_LATEX_ERRORS = (cat $(OUTPUT_DIR)/$(PAPER).log | grep '^[^: ]*:[^: ]*:' || exit 0)
PRINT_LATEX_WARNINGS = (cat $(OUTPUT_DIR)/$(PAPER).log | grep -i 'latex warning' || exit 0)
PRINT_BIBTEX_WARNINGS = (cat $(OUTPUT_DIR)/*.blg | grep '^Warning' | sort | uniq > $(BIB_OUT_FILE) || exit 0)
PRINT_BIBTEX_NOTE = if [ -s $(BIB_OUT_FILE) ]; then \
                    echo "$(NOTE_LABEL)Bibliography warnings written to '$(BIB_OUT_FILE)'."; fi

#formats
NORM=
BOLD=
PS2PDF_LABEL   =[ps2pdf   ] 
DVIPS_LABEL    =[dvips    ] 
LATEX_LABEL    =[latex    ] 
BIBTEX_LABEL   =[bibtex   ] 
NOTE_LABEL     =[note     ] 
MAKEINDEX_LABEL=[makeindex] 
RM_LABEL       =[rm       ] 

SHELL:=/bin/bash

all: $(OUTPUT_DIR)/$(PAPER).pdf

show: $(OUTPUT_DIR)/$(PAPER).pdf
	@evince $(OUTPUT_DIR)/$(PAPER).pdf &

$(OUTPUT_DIR)/$(PAPER).pdf: $(TEXT_DIR)/$(PAPER).tex                      \
                            $(shell find $(TEXT_DIR) -regex "[^.]*.tex")  \
                            $(shell find $(TEXT_DIR) -regex  "[^.]*.bib") \
                            $(shell find $(STYLE_DIR) -regex "[^.]*.tex") \
                            $(shell find $(FIGURE_DIR) -name "*.pdf") 
	@mkdir -p $(OUTPUT_DIR)

	@echo "$(LATEX_LABEL)Performing initial latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

	@echo "$(BIBTEX_LABEL)Processing bibliography..."
	@BIBINPUTS=$(BIB_PATH) \
	 BSTINPUTS=$(BST_PATH) \
		bibtex $(BIBTEX_OPTS)  $(OUTPUT_DIR)/$(PAPER) | grep -v "^Warning"; \
		if [ $${PIPESTATUS[0]} != 0 ]; then \
			rm -f $@ && exit 1; \
		fi 
	@-$(PRINT_BIBTEX_WARNINGS)
	@-$(PRINT_BIBTEX_NOTE)

#	@echo "$(MAKEINDEX_LABEL)Building index..."
#	@makeindex $(MAKEINDEX_OPTS) $(OUTPUT_DIR)/$(PAPER).idx || \
#		(rm -f $@ && exit 1)

	@echo "$(LATEX_LABEL)Performing secondary latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

#	@echo "$(LATEX_LABEL)Performing ternary latex..."
#	@TEXINPUTS=$(TEX_PATH) \
#		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
#			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

	@echo "$(LATEX_LABEL)Performing final latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)
	@-$(PRINT_LATEX_WARNINGS)

clean:
	@echo '$(RM_LABEL)Cleaning project...'
	@rm -fr bib-issues main.aux main.blg main.log main.out main.pdf

